PhantomCall: Evading ML Malware Detectors via Function Call Graph Perturbation

Prior adversarial attacks on Windows PE malware detectors target raw bytes, PE headers, or intra-function control-flow graphs, leaving the function call graph (FCG) unexplored as an attack surface. Yet the FCG structure is an important feature in graph-based malware detectors. We present Phan- tomCall, a black-box attack that perturbs the FCG of Windows PE malware by injecting fully executable dummy functions at targeted call sites, adding new nodes and edges to both the CFG and FCG while preserving program semantics. We pair this structural perturbation with classifier-guided search and tunable injection parameters, effective across three archi- tecturally distinct classifiers. Evaluated on a 2025-collected Windows malware corpus against MalConv (raw-byte CNN), MalGraph (graph-based GNN), and SAFE+GNN (pure FCG GNN trained from scratch on a 2024 corpus) at two FPR thresholds, the best PhantomCall variant achieves 85-100% attack success rate across all configurations, exceeding prior state-of-the-art by up to 14.78 percentage points on MalGraph and 95.5 percentage points on SAFE+GNN, and generating evasive variants up to 2.9x faster on average across all targets. For MalConv and MalGraph, the majority of evasions require only a single call site modification, and 86-97% of evaluated evasive variants preserve the original malicious behavior in sandbox-based semantic testing across all configurations.

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}\label{sec:appendix}
% 
Generative AI tools were used to assist with implementation, debugging, and paper editing during the development of this work. All AI-generated artifacts were reviewed by the authors, who take full responsibility for the accuracy and correctness of the paper's content.

==> sections/ethics.tex <==
\section{Ethics Considerations}\label{sec:ethics}
All experiments were conducted on known malware samples from MalwareBazaar under a static-only pipeline. No adversarial variants were executed outside isolated environments, distributed, or publicly released. The generated adversarial variants are not publicly released, and we will share only cryptographic hashes of the original samples to enable reproducibility. This research does not involve human subjects and does not require IRB approval.

==> sections/overview_old_LLM_Driven_SEMNOP_GENERATION.tex <==
\section{Introduction}\label{sec:overview}
\noindent In this section, we define our problem formally and state the challenges and approach to solutions to those challenges.

\subsection{Challenges \&  Solution Outline}
\noindent We now discuss the main challenges and the solution approaches that guided us to design \system{}.

\noindent \textbf{(C1) Large Search Space of Attack Sites in Assembly Code} 

% Recent advancements in Large Language Models(LLMs) have significantly advanced their abilities for code generation for a variety of different programming tasks across multiple languages thanks to the vast amount of open-source code as part of their training corpus.[]. To prevent the misusage of these models, modern LLMs undergo ethical alignment procedures during training to avoid generating harmful content such as malware from scratch ~\cite{ouyang2022training, bai2022training} However, determined adversaries may use LLMs to generate functional components of malware and assemble them to create malicious programs. This approach, though, requires advanced prompt engineering that targets the specific malware type being created and would not generalize for producing a large number of adversarial malware variants in a short amount of time. In addition to this, successfully crafting malware in such a way demands a deep knowledge about the malware being designed, creating a steep barrier for novice attackers without significant expertise. These challenges highlight the complexity involved in bypassing LLM safeguards to facilitate large-scale malware generation without explicitly training models for malicious purposes.

%Something new should be here

\looseness  = - 1
\noindent \textbf{(A1)}
TBD
% LLM Code generation with assembly.} To address the challenges outlined in \textbf{C1}, we decided to leverage the code generation capability of LLMs but not for generating malware as a whole or functional components, rather focusing on intermediate representations. Various design choices exist in this space, including Compiler Intermediate Representations (IR) such as LLVM-IR and assembly code. Although there are datasets such as ~\cite{paul2024ircoder, grossman2023compile} for LLVM-IR and models such as Meta's recently released \cite{cummins2024meta}, these are more tailored for compiler optimization and disassembly rather than general instruction-based code generation through prompts without substantial model retraining or fine-tuning.  Thus, we opted for assembly code generation, specifically in a simplified format like NASM, to create diverse and intricate shellcodes and use them with malware binaries to produce evasive variants in a large-scale setting. 


\noindent \textbf{}
% A pertinent question is why not utilize existing LLMs that are apt at handling source code for refactoring or transforming existing malware at the assembly code level?  Unlike source code, assembly code has lower information density, and small-sized source code instructions may span several assembly instructions ~\cite{anonymous2024nova}. This characteristic of assembly code poses a significant challenge for LLMs regarding reasoning and understanding the language. Current LLMs specializing in source code ~\cite{zhu2024deepseek, roziere2023code, codestral} still struggle to work and reason with the language despite assembly code in their training corpus. Specialized LLMs for assembly code such as ~\cite{anonymous2024nova, tan2024llm4decompile, cummins2024meta} are fine-tuned on specific assembly tasks such as decompilation and optimization, limiting their general applicability for prompt-based assembly code refactoring without additional training. Prior work ~\cite{lucas2021malware, pappas2012smashing} has focused on transforming malware assembly code with in-place replacement of instructions and code displacement attacks following different strategies. However, applying these techniques using LLMs is impractical due to context limitations that hinder the model's ability to handle entire binary files containing hundreds or thousands of instructions. Although we can attempt to process the binary files' assembly counterparts by processing small chunks of assembly code to perform transformations, it would be time-intensive and prone to errors given current context window limitations. Moreover, most commercial and academic disassembler tools produce disassembled code that is far from what an assembler would process\cite{wang2015reassembleable}, which in turn would make it extremely difficult for an LLM to understand and process such assembly codes without additional fine-tuning as such non-trivial languages are usually not present in the training corpus of these models.

\noindent \textbf{(A2)} 
% LLM generated assembly shellcode injection to malware binaries.} As we observe the challenge of assembly code transformation with LLM, we propose leveraging LLMs to generate assembly code that can be injected as shellcode directly into Windows malware binaries instead of assembly code transformation. By selecting assembly code as the intermediate representation for generated code and targeting malware binaries instead of source codes, we get to utilize LLM code generation capability as well as circumvent the limitation that comes with assembly code transformations. Effective prompt engineering allows us to harness the capability of instruction-tuned models without further fine-tuning. This approach also mitigates the issue of limited context window problems of LLMs when dealing with byte/binary modification or addition directly on malware PE files.

\noindent \textbf{(C3) Informed Semantic NOPS selection}
% Hallucination has been a well-studied problem in NLP and LLM ~\cite{ji2023survey,huang2023survey} and is also relevant to code generation. The study by ~\cite{liu2024exploring} systematically analyzes code hallucination in LLMs and provides key insights into why hallucination and code functionality may be correlated. One of the most notable categorizations of the code hallucination problem is intent-conflicting hallucination~\cite{liu2024exploring}, where the authors term it as generated content that deviates from the user’s intent with a relatively small semantic correlation. This underscores the non-deterministic nature of LLMs, which may not always adhere to precise instructions for code generation. In our context of the problem of large-scale adversarial malware generation by addressing both challenges \textbf{C1} and \textbf{C2}, we discuss the approach to use assembly code generation with prompt engineering to generate sophisticated shellcode for injection to malware to fool classifiers and virus detection engines. However, the prevalence of hallucination and erroneous code generation creates an impediment to the process. For instance, one of the key requirements for generated assembly code is to properly preserve the registers that are used in the generated code snippet and then restore them in order. Failure to adhere to these guidelines can result in injected code that causes the malware to malfunction or crash, thereby nullifying its functionality. Thus, balancing the creative potential of LLMs in generating diverse and sophisticated shellcode code while maintaining the integrity and functionality of existing malware is a formidable challenge.

\noindent \textbf{(A3) LLM Self-error correction strategy and designing tester/oracle program} To tackle \textbf{C3}, we design an LLM-based error correction mechanism that is fully automated in the code generation framework. This would enable the model to self-correct syntactical, logical, and register preservation errors before we use the code snippets as shellcodes for injection. In addition to this, before injecting the code into malware, we manually design and use a tester( or several testers) program to verify if the generated code snippet is safe to be injected into malware without harming the regular execution flow of the code. In the evaluation section [ place exact evaluation section here ], we demonstrate the efficacy of our design choices for each step by conducting detailed ablation studies.


\textbf{The following challenge is tentative and is to be determined if indeed LLM generated shellcode combined with their existing search is very slow.}

\noindent \textbf{(C4) Speeding up Search Space with LLM inference.}
The adversarial malware search space is discrete and infinite \cite{ling2024wolf} and combining Monte Carlo Tree Search for the context of finding optimal call instruction for call-based redividing attacks\cite{ling2024wolf} and LLM-based shellcode generation can be quite computationally expensive and would drastically slow down the generation of large scale adversarial malware variants. 

\noindent \textbf{(A4) Using simpler search with LLM based code generation}. To tackle \textbf{C4}, we use simpler search methods such as Beam Search, and Simulated Annealing to find the optimal cfg transformation that is capable of evading malware detectors while also leveraging our robust LLM-based assembly code generation framework to generate sophisticated shellcode.
